A Simple Stochastic Differential Equation with Discontinuous Drift

In this paper we study solutions to stochastic differential equations (SDEs) with discontinuous drift. We apply two approaches: The Euler-Maruyama method and the Fokker-Planck equation and show that a candidate density function based on the Euler-Maruyama method approximates a candidate density function based on the stationary Fokker-Planck equation. Furthermore, we introduce a smooth function which approximates the discontinuous drift and apply the Euler-Maruyama method and the Fokker-Planck equation with this input. The point of departure for this work is a particular SDE with discontinuous drift.

==> eptcsdata.tex <==
\providecommand{\firstpage}{109}
\providecommand{\publicationstatus}{Bortolussi, Bujorianu, Pola (Eds.): HAS 2013\\
EPTCS 124, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.124.11}{10.4204/EPTCS.124.11}}
\pdfoutput=1

